GS-LIVO: Real-Time LiDAR, Inertial, and Visual Multi-sensor Fused Odometry with Gaussian Mapping

In recent years, 3D Gaussian splatting (3D-GS) has emerged as a novel scene representation approach. However, existing vision-only 3D-GS methods often rely on hand-crafted heuristics for point-cloud densification and face challenges in handling occlusions and high GPU memory and computation consumption. LiDAR-Inertial-Visual (LIV) sensor configuration has demonstrated superior performance in localization and dense mapping by leveraging complementary sensing characteristics: rich texture information from cameras, precise geometric measurements from LiDAR, and high-frequency motion data from IMU. Inspired by this, we propose a novel real-time Gaussian-based simultaneous localization and mapping (SLAM) system. Our map system comprises a global Gaussian map and a sliding window of Gaussians, along with an IESKF-based odometry. The global Gaussian map consists of hash-indexed voxels organized in a recursive octree, effectively covering sparse spatial volumes while adapting to different levels of detail and scales. The Gaussian map is initialized through multi-sensor fusion and optimized with photometric gradients. Our system incrementally maintains a sliding window of Gaussians, significantly reducing GPU computation and memory consumption by only optimizing the map within the sliding window. Moreover, we implement a tightly coupled multi-sensor fusion odometry with an iterative error state Kalman filter (IESKF), leveraging real-time updating and rendering of the Gaussian map. Our system represents the first real-time Gaussian-based SLAM framework deployable on resource-constrained embedded systems, demonstrated on the NVIDIA Jetson Orin NX platform. The framework achieves real-time performance while maintaining robust multi-sensor fusion capabilities. All implementation algorithms, hardware designs, and CAD models will be publicly available.

==> arxiv_supply.tex <==
% Supplemental Materials
% \let\proof\relax
% \let\endproof\relax
% \let\example\relax
% \let\endexample\relax
% \let\labelindent\relax
% \let\algorithm\relax

% \usepackage{makecell}
% \usepackage{times}
% \usepackage[pdftex]{graphicx}
% \usepackage{subfigure}
% \usepackage{amsmath,amssymb,amsopn,amstext,amsfonts}
% \usepackage{cancel}
% \usepackage[space]{cite}
% \usepackage{soul}
% \usepackage{cuted}
% \usepackage{caption}
% \usepackage{lipsum,multicol}
% \usepackage{stfloats}
% \usepackage{ulem}
% \everymath{\displaystyle}
% \usepackage{booktabs}
% \usepackage{threeparttable}
% \usepackage{amsthm}
% \usepackage{xfrac}
% \usepackage{balance}
% \usepackage{color}
% \usepackage{mathtools}
% \DeclareMathOperator*{\med}{med}
% \usepackage{tabularx}
% \usepackage{bm}
% \usepackage{diagbox}
% \usepackage{float}
% \usepackage{epstopdf}
% \usepackage{url}
% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage{tikz}
% \usepackage{tablefootnote}
% \usepackage{wrapfig}
% \usepackage{graphicx}
% \usepackage{siunitx} %\usepackage[linkcolor=black,citecolor=black,urlcolor=black,colorlinks=true]{hyperref}

\clearpage
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{1}
\setcounter{section}{0}%
\setcounter{subsection}{0}%
\setcounter{subsubsection}{0}%
\setcounter{paragraph}{0}%
% \IEEEoverridecommandlockouts
% \bibliographystyle{support/IEEEtran}
\onecolumn

% \title{Supplementary Material for FAST-LIVO2: Fast, Direct LiDAR-Inertial-Visual Odometry}
% \author{Chunran Zheng, Wei Xu, Zuhao Zou, Tong Hua, Chongjian Yuan, Dongjiao He, Bingyang Zhou, Zheng Liu, Jiarong Lin, Fangcheng Zhu, Yunfan Ren, Rong Wang, Fanle Meng, Fu Zhang % <-this % stops a space  
% }
\begin{center}
	\textbf{\large Supplementary Material for GS-LIVO}
\end{center}
% \renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thetable}{S\arabic{table}}
% \begin{document}
% \maketitle
\section*{I. System Module Validation}\label{subsec:module_valid}
In this section, we conduct a thorough validation of the essential modules of our system. These modules include affine warping, normal refinement, reference patch update, on-demand raycasting the affine warping, normal refinement, {reference patch update}, on-demanding raycasting query, exposure time estimation, {and ESIKF sequential update utilizing the FAST-LIVO2 private dataset and MARS-LVIG dataset.}
\subsection*{A. Evaluation of Affine Warping}\label{subsubsec:affine_warp}
{In this experiment, we aim to comprehensively evaluate the various affine warping effects based on the {constant depth assumption} (a common technique utilized in semi-dense methods), the plane prior from point clouds, and the refined plane normal of our proposed system (denoted as {``Constant depth"}, ``Plane prior", and ``Plane normal refined“, respectively). To achieve this, we compare the mapping results and drift metrics of the three methods on ``CBD Building 02" and ``Office Building Wall".}


